PhyPlan: Generalizable and Rapid Physical Task Planning with Physics Informed Skill Networks for Robot Manipulators

Given the task of positioning a ball-like object to a goal region beyond direct reach, humans can often throw, slide, or rebound objects against the wall to attain the goal. However, enabling robots to reason similarly is non-trivial. Existing methods for physical reasoning are data-hungry and struggle with complexity and uncertainty inherent in the real world. This paper presents PhyPlan, a novel physics-informed planning framework that combines physics-informed neural networks (PINNs) with modified Monte Carlo Tree Search (MCTS) to enable embodied agents to perform dynamic physical tasks. PhyPlan leverages PINNs to simulate and predict outcomes of actions in a fast and accurate manner and uses MCTS for planning. It dynamically determines whether to consult a PINN-based simulator (coarse but fast) or engage directly with the actual environment (fine but slow) to determine optimal policy. Given an unseen task, PhyPlan can infer the sequence of actions and learn the latent parameters, resulting in a generalizable approach that can rapidly learn to perform novel physical tasks. Evaluation with robots in simulated 3D environments demonstrates the ability of our approach to solve 3D-physical reasoning tasks involving the composition of dynamic skills. Quantitatively, PhyPlan excels in several aspects: (i) it achieves lower regret when learning novel tasks compared to the state-of-the-art, (ii) it expedites skill learning and enhances the speed of physical reasoning, (iii) it demonstrates higher data efficiency compared to a physics un-informed approach.

==> sections/evaluation-results-big.tex <==
Through our evaluation, we first investigate the physics-informed skill model for the ability to predict object motions during dynamic interactions (such as sliding, hitting, throwing, etc.) and the data efficiency achieved compared to conventional physics-uninformed time series models. Then, we study the degree to which the proposed planner can learn to perform a physical reasoning task requiring a composition of learnt skills. Finally, we show, qualitatively, a simulated Franka Emika Robot performing the tasks.

\begin{figure*}[tb]
\centering
\def\imgwidth{0.245\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/pendulum.png}
\includegraphics[width=\imgwidth]{Images/result/Task/wedge.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding_bridge.png}
\caption{\textbf{Task Solving Accuracy:} Comparing the performance of our approach and the baselines based on the minimum regret achieved vs the number of actions taken in the evaluation phase for each task. Lower is better. Our approach consistently beats the baselines.}
\label{fig:regret-results}
\vspace{3mm}
\end{figure*}

\subsection{Experimentation Setup}

\paragraph{Virtual Skill Learning:} We deploy Isaac Gym ~\cite{nvidia2022isaacgym}, a physics simulator and reinforcement learning framework for training robots and skill learning. The task involves learning physical skills like swinging, sliding, throwing, hitting and bouncing (Figure \ref{fig:skill-learning}). Each task is simulated, and a Physics-Informed Skill model is trained over the data received. Consider the case of throwing a ball in the simulator, which provides velocity-displacement pair values of the projectile at different time instances as training input to the model. Similar experiments are done for each skill.

\paragraph{Perception-based Skill Learning:} We also developed a perception-based pipeline to infer the object state directly from RGB-D data to replicate real lab-based settings. The experimentation scene in the simulator is captured via an inbuilt depth camera, which provides time series images of the experiment. On the gathered image dataset, segmentation techniques involving a combination of unsupervised detection methods like Segment Anything~\cite{kirillov2023segment}, Grounding Dino~\cite{liu2023grounding} and traditional methods like edge detection are used for object detection.  

\subsection{Evaluation of Learnt Skills} 

We evaluate the prediction accuracy of the proposed physics-informed skill network on simulation data and the physical parameter estimation in the unknown environment. 

\textbf{Skill model accuracy} There are two types of proposed models based on the data collection regime employed: \textit{Physics-Informed Neural Network} (Figure \ref{fig:network_arch}) a) \textit{with perception} and b) \textit{without perception}. For training the PINN model, actual data points and collocation or pseudo points (4 times the data points) are considered for optimising physics-based loss. The proposed models are compared against standard Feedforward network (NN) (same architecture as PINN but with only data-driven loss) (a) with perception and (b) without perception. Figure \ref{fig:skill-model} indicates that the model with only physics loss performs poorly, and incorporating physics governing equations with the data loss allows stronger generalisation and improved data efficiency compared to general physics-uninformed time series models. PINN without perception is the most efficient skill-learning model. Although its performance degrades with perception-based training due to inherent noise in the data, PINN performs better than Perception NN.

\textbf{Unknown parameters and robustness} PINN-based skill models are particularly useful and efficient when the inherent variables of the environment are unknown, as depicted by Figure \ref{fig:unknown}. PINN model is data efficient, which is highlighted by the fact that it requires very few data points (approximately 700-1000 points) to accurately determine the actual $\mu$ value. Note even though the perception-based approach is inherently noisy, there is a meagre difference between predicted $\mu$ values by PINN models with and without perception, depicting the robustness of our perception-based approach.

\subsection{Evaluation on Physical Reasoning Tasks}
\textbf{Dataset and Baselines}
We created a benchmark data set composed of four tasks: Launch, Slide, Bounce, and Bridge, which require the robot to use physical skills sequentially to attain the goal. For example, the Bridge task requires a dynamic object like a ball to be positioned into a goal region. The task requires chaining multiple interactions with objects. The robot can interact with the environment multiple times, resetting the dynamic object after each complete rollout. Within each trial, the robot can set the objects in the desired configuration before releasing the dynamic object. The robot only observes an image of the scene. 
%
We also implemented the following baselines for comparisons:
(i) \emph{Random policy:} actions sampled uniformly at random, 
(ii) \emph{DQN-n-Simple:} a DQN baseline from \cite{bakhtin2019phyre} trained using random contexts (images) and random actions. The policy is extracted by selecting the highest scoring actions by sampling $10,000$ actions randomly and
(iii) \emph{DQN-n-Adapted}: similar to (ii) except for using a Gaussian Process to regress over rewards from prior rollouts.

\begin{figure*}[tb]
\centering
\def\imgwidth{0.33\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_Random_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Simple_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Adaptive_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_Without_GP-UCB_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_With_GP-UCB_wedge_2.PNG}
\caption{\textbf{Visual Adaption of Reward Model:} Showing the coordinates of the goal and the ball for 50 iterations. Online Learning explores the action space exhaustively and converges to the optimal action by capturing the systematic errors made by the pre-trained models.}
\label{fig:online-learning}
\end{figure*}

\textbf{Task Learning Efficacy.}
We built two versions of our model called \emph{PhyPlan with perception} and \emph{PhyPlan without perception}. The former uses perception-based PINN models and extracts the goal and ball positions from the task image. The latter uses PINN models without perception and obtains goal and ball positions directly from the simulator. Figure \ref{fig:regret-results} illustrates the task learning efficiency measured as regret, defined in Section \ref{sec:problem-formulation}. The lower the regret, the better the performance. Both versions of PhyPlan achieve lower regret than the baselines. As the task complexity increases, the difference between PhyPlans' performance and the baselines widens. For instance, PhyPlan performs close to the baselines in the Sliding task, whereas it outperforms baselines by a high margin in the Bridge task. Further, \emph{PhyPlan without perception} generally performs better than \emph{PhyPlan with perception} because of the inherent noise in the Perception-based skill models and the errors in detecting the goal and ball positions.
Figure \ref{fig:dqn-comp} shows a qualitative comparison between PhyPlan and DQN-Adaptive in the \emph{Bridge} task. PhyPlan demonstrates the capability of long-horizon reasoning in substantially less number of actions/trials.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Images/result/Task/Time.png}
    \caption{PhyPlan's runtime is manifold less than that of planner without Physics-Informed skill models.}
    \label{fig:time-results}
\end{figure}
Further, Figure \ref{fig:time-results} compares our approach with its variant, which uses a full simulation engine during training instead of learnt skills. The results indicate the benefit of using the learnt model during planning. The proposed approach achieves significant runtime gains (reducing calls to the time-consuming physics engine) while achieving better task-solving ability.

\textbf{Adaption of Reward Model.}
We also evaluated the effectiveness of GP-UCB in adapting to the task execution environment, beginning with the pre-trained Physics-Informed Skill Models. Figure \ref{fig:online-learning} illustrates the final positions where the dynamic object (the ball) lands relative to the goal after the robot performs the \emph{Bounce} task. The Random model spans the whole action space, the \emph{DQN-Simple} model is skewed as it does not learn online, the \emph{DQN-Adaptive} model converges to the goal position in later iterations, \emph{PhyPlan without GP-UCB} does not explore as it does not learn the prediction error, and \emph{PhyPlan with GP-UCB} learns the prediction error to converge to the goal position quickly. Further, \emph{PhyPlan with GP-UCB} appears to learn more systematically, exploring and refining within a confined action space.

Figure \ref{fig:task-plan} demonstrates a simulated Franka Emika robot learning to perform the tasks. The robot interacts with the objects using crane grasping with a task space controller for trajectory tracking. The Figure shows the robot learning (i) the ball's release height and the wedge's pose in \emph{Bounce} task; (ii) the pendulum's plane and angle in the \emph{Launch} and the \emph{Bridge} tasks; (iii) the bridge's pose in the \emph{Bridge} task for the ball or puck to fall into the goal region. The policy is learned jointly for all objects, and the actions are delegated to the robot with the desired object in its kinematic range. Once the robots position the tools, the ball or the pendulum is dropped. Further, note that the robot learns to use the bridge effectively; a physical reasoning task reported earlier \cite{allen2020rapid} to be challenging to learn for model-free methods, highlighting the PhyPlan's adaptability to long-horizon tasks. The results indicate the ability to generalise to new goal locations by using objects in the environments to aid task success.
%The results are best viewed as a video submitted as a multi-media supplement to this manuscript. 

\begin{figure*}[t]
\centering
\def\imgwidth{0.33\linewidth}
    \setcounter{subfigure}{0}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-1.png}
        \caption{DQN-Adaptive: Action 1}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-4.png}
        \caption{DQN-Adaptive: Action 4}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-11.png}
        \caption{DQN-Adaptive: Action 11}
    \end{subfigure}
    \setcounter{subfigure}{0}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/1.png}
        \caption{PhyPlan: Action 1}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/2.png}
        \caption{PhyPlan: Action 2}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, height=0.687\linewidth, frame]{Images/result/Qualitative/Bridge/4.png}
        \caption{PhyPlan: Action 4}
    \end{subfigure}
    \caption{\textbf{Comparing PhyPlan with DQN-Adaptive.} Showing the actions performed by DQN-Adaptive vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use the bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
    \label{fig:dqn-comp}
\vspace{3mm}
\end{figure*}

\begin{figure*}[tb]
\centering
\def\imgwidth{0.19\linewidth}
% \renewcommand*{\thesubfigure}{\alph{subfigure}}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/1_Initial_State.PNG}
        \caption{\fontsize{7}{8}\selectfont Initial State}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/2_Pick_bob.PNG}
        \caption{\fontsize{7}{8}\selectfont Pick the bob}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/3_Adjusting_Plane.PNG}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/4_Adjusting_Angle.PNG}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/5_Final_State.PNG}
        \caption{\fontsize{7}{8}\selectfont Final State}
    \end{subfigure}

\vspace{5mm}

    \setcounter{subfigure}{0} 
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/1_init_state.png}
        \caption{\fontsize{7}{8}\selectfont Initial State}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/2_orient_wedge.png}
        \caption{\fontsize{7}{8}\selectfont Orienting Wedge}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/3_pick_ball.png}
        \caption{\fontsize{7}{8}\selectfont Picking the Ball}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/4_release_ball.png}
        \caption{\fontsize{7}{8}\selectfont Releasing the Ball}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/5_final_state.png}
        \caption{\fontsize{7}{8}\selectfont Final State}
    \end{subfigure}

\vspace{5mm}

    \setcounter{subfigure}{0} 
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge Plan/1_init_state.png}
        \caption{\fontsize{7}{8}\selectfont Initial State}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge Plan/2_place_bridge.png}
        \caption{\fontsize{7}{8}\selectfont Placing Bridge}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge Plan/3_adjust_plane.png}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge Plan/4_adjust_angle.png}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge Plan/5_Final_state.png}
        \caption{\fontsize{7}{8}\selectfont Final State}
    \end{subfigure}

\vspace{5mm}

    \setcounter{subfigure}{0} 
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/1_init_state.png}
        \caption{\fontsize{7}{8}\selectfont Initial State}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/2_adjust_plane.png}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/3_adjust_angle.png}
        \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, height=0.67\linewidth, frame]{Images/result/Qualitative/Slide Plan/4_release_bob.png}
        \caption{\fontsize{7}{8}\selectfont Releasing the Pendulum}
    \end{subfigure}
    \begin{subfigure}{\imgwidth}
        \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/5_final_state.png}
        \caption{\fontsize{7}{8}\selectfont Final State}
    \end{subfigure}

\vspace{5mm}

\caption{\textbf{Simulated Robot Demonstrations.} Physical reasoning tasks learnt by a robot. See videos submitted in the supplementary material.   
\textbf{LAUNCH:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to throw the ball into the box.
\textbf{BOUNCE:} After 3 actions and 10 PINN-rollouts per action, the robot learns to align the wedge correctly and releases the ball at an appropriate height to bounce it into the box.
\textbf{BRIDGE:} After 5 actions and 20 PINN-rollouts per action, the robot learns to place the bridge in the path of the box and releases the pendulum from the correct location to slide the box to the goal.
\textbf{SLIDE:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to slide the puck to the goal.
}
\label{fig:task-plan}
\end{figure*}


==> sections/evaluation-results-more.tex <==
Through our evaluation, we investigate i) the ability and efficiency of physics-informed skill networks to model different skills and adapt to unknown physical parameter settings, ii) the degree to which our approach can generalize to solving unseen tasks using a composition of learnt skills and iii) the qualitative insights and performance of Franka Emika Robot on different physical reasoning tasks.

\setcounter{figure}{3}

% \begin{figure*}[t]
%     \centering
%     \begin{minipage}[t]{.57\textwidth}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/Wedge_3.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_0.5.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_0.75.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_1.png}}
%         \end{subfigure}
%         \caption{Showing position of the ball predicted by a chain of skill networks at various time steps at a gap of 0.01 seconds ($t_{query}$) in \emph{Bounce} Task. The agent varies the initial drop height (here $0.5, 0.75\ and\ 1.0$) and expects the final resting position of the ball to evaluate the reward.}
%         \label{fig:bounce_chain}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{.42\textwidth}
%         \includegraphics[width=\linewidth]{Images/result/Qualitative/DQN-vs-PhyPlan_Bridge.PNG}
%         \caption{\textbf{Comparing PhyPlan with DQN-Adaptive.} Showing the actions performed by DQN-Adaptive vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use the bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
%         \label{fig:dqn-comp}
%     \end{minipage}
% \end{figure*}

% \begin{figure*}[tb]
% \centering
% \def\imgwidth{0.325\linewidth}
%     \setcounter{subfigure}{0}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-1.png}
%         \caption{DQN-Adaptive: Trial 1}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-4.png}
%         \caption{DQN-Adaptive: Trial 4}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-11.png}
%         \caption{DQN-Adaptive: Trial 11}
%     \end{subfigure}
%     \setcounter{subfigure}{0}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/1.png}
%         \caption{PhyPlan: Trial 1}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/2.png}
%         \caption{PhyPlan: Trial 2}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.687\linewidth, frame]{Images/result/Qualitative/Bridge/4.png}
%         \caption{PhyPlan: Trial 4}
%     \end{subfigure}
%     \caption{\textbf{Comparing PhyPlan with DQN-Adaptive.} Showing the actions performed by DQN-Adaptive vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use the bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
%     \label{fig:dqn-comp}
% % \vspace{3mm}
% \end{figure*}

% \begin{figure*}[tb]
% \centering
% \def\imgwidth{0.33\linewidth}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_Random_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Simple_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Adaptive_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_Without_GP-UCB_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_With_GP-UCB_wedge_2.PNG}
% \caption{\textbf{Visual Adaption of Reward Model:} Showing the coordinates of the goal and the ball for 50 iterations. Online Learning explores the action space exhaustively and converges to the optimal action by capturing the systematic errors made by the pre-trained models.}
% \label{fig:online-learning}
% \end{figure*}

%% Skill network evaluation
\subsection{Physical Skill Network Evaluation} 
%
We evaluate the prediction accuracy of the proposed physics-informed skill networks on simulation data and the physical parameter estimation in unknown environments. 
%
Figure \ref{fig:skill-model} indicates that the model with \emph{only physics loss} performs poorly due to noise in the system. Figure \ref{fig:data-eff} shows PINN models requires less data than their NN counterpart. Therefore, incorporating physics governing equations with the data loss allows stronger generalisation and improved data efficiency compared to general \emph{physics-uninformed or data only} time series models.
%
 Figure \ref{fig:skill-model} shows the skill networks trained with or without bounding boxes. We also compare the standard Feed forward neural network  (same architecture but with only data-driven loss) (a) with perception and (b) without perception. PINN without perception is the most efficient skill-learning model. Although performance degrades with perception-based training due to inherent noise in data, PINN still performs better the baseline.

\begin{figure}[h]
    \centering
        \includegraphics[width=0.5\linewidth]{Images/result/Quantitative/bar_plot_final.png}
        \includegraphics[width=0.48\linewidth, height=0.425\linewidth]{Images/result/Quantitative/bar_col_plot_final.png}
        \caption{\textbf{Skill Network Accuracy.} Comparing prediction loss on validation dataset. \textbf{Left:} PINN (Physics and Data) without perception performs better than other networks due to the guiding physics and exact data. Physics has less impact in perception-based pipeline due to inherent noise. \textbf{Right:} NN without perception performs better than NN with perception.}
        \label{fig:skill-model}
        % \vspace{-1mm}
\end{figure}

\begin{figure}[h]
    \centering
    \subfloat[Throwing Skill]{\includegraphics[width=0.33\linewidth]{Images/result/PINN/throwing_data_final.png}}
    \subfloat[Sliding Skill]{\includegraphics[width=0.33\linewidth]{Images/result/PINN/sliding_data_final.png}}
    \subfloat[Swinging Skill]{\includegraphics[width=0.33\linewidth]{Images/result/PINN/swinging_data_final.png}}
    \vspace{2mm}
    \caption{\textbf{Data Efficiency.} PINN displays superior data efficiency over NN, highlighted by lower validation MSE loss for the same Training Data size in various initial settings.}
    \label{fig:data-eff}
    % \vspace{3mm}
    \vspace{-2mm}
\end{figure}

\begin{figure}[h] 
\centering
    \includegraphics[width=0.51\linewidth]{Images/result/PINN/sliding_unknown_new.png}
    \includegraphics[width=0.47\linewidth]{Images/result/PINN/distance_plot.png}
    \caption{\textbf{Left: Unknown Parameter} Estimating $\mu$ in \textit{sliding skill}, PINN-based approach achieves a relatively low error within a few time steps. \textbf{Right:} \emph{Generalizing} on variable parameters, PINN is able to accurately predict trajectory of box sliding on surface with variable $\mu$, hence it is efficient.}
    \label{fig:unknown}
    \vspace{-2mm}
\end{figure}

% Generalization to environments with unknown physical parameters. 
Next, we evaluate the degree to which the skill networks can generalize to environment without \emph{a-priori} knowledge of physical parameters during object interactions. Figure \ref{fig:unknown}(a) indicates the the skill networks recovers the unknown physical parameters (coefficient of friction) with increasing training data points during a single roll out. The model recovers recovers the latent parameter within $100$ time steps within a single roll out. Figure \ref{fig:unknown}(b) shows the skill network generalising conditioned on the inferred physical parameter. 


%% Task Level Evaluation
\subsection{Evaluation on Physical Reasoning Tasks}


We implemented the following baselines for comparisons:\footnote{As noted in~\cite{bakhtin2019phyre} policy based learners: A2C~\cite{mnih2016asynchronous} and PPO~\cite{schulman2017proximal} perform poorly as compared to random baseline due to poor training stability hence Deep Q Networks and Random baselines are preferred for evaluation.}
(i) \emph{Random policy:} actions sampled uniformly at random, 
(ii) \emph{DQN-No Adapt:} a DQN baseline from \cite{bakhtin2019phyre} trained using random contexts (images) and random action, reward pairs. The policy is extracted by selecting the highest scoring actions by sampling $10,000$ actions randomly and
(iii) \emph{DQN}: similar to (ii) except, it uses a Gaussian Process to regress over rewards from prior rollouts, as we do in PhyPlan.

\setcounter{figure}{7}
\begin{figure*}[tb]
\centering
\def\imgwidth{0.245\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/pendulum.png}
\includegraphics[width=\imgwidth]{Images/result/Task/wedge.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding_bridge.png}
\caption{\textbf{Performance on Unseen Tasks:} Comparing our approach and the baselines based on the minimum regret achieved vs the number of trials taken in the evaluation phase for each task. Lower is better. \emph{DQN - No Adapt} does not learn the adapt online. \emph{DQN} and \emph{PhyPlan} both use Gaussian Process for online learning. PhyPlan achieves the lowest regret consistently.}
\label{fig:regret-results}
% \vspace{-1mm}
\end{figure*}

\setcounter{figure}{8}
\begin{figure*}[tb]
\centering
\def\imgwidth{0.195\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_Random_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN - No Adapt_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan - No Adapt_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_wedge_2.png}
\caption{\textbf{Effect of GP-based adaptation of reward distribution:} Showing the ball's coordinates relative to the goal for 50 iterations. Online Learning explores the action space exhaustively and converges to the optimal action by capturing the systematic errors made by the pre-trained skill networks.}
\label{fig:online-learning}
% \vspace{3mm}
\end{figure*}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/1.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/2.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/3.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/4.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/5.png}
    \caption{\textbf{Robot performing Launch Task.} After 2 trials and 10 PINN-rollouts per trial, the robot learns to correctly align the pendulum's plane and angle to throw the ball into the box.}
    \label{fig:pendulum-plan}
\vspace{-2mm}
\end{figure*}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/1.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/2.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/3.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/4.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/5.png}
    \caption{\textbf{Robot performing Demonstrations for Bridge Task.} After 5 trials and 20 PINN-rollouts per trial, the robot learns to place the bridge in the path of the box and releases the pendulum from the correct location to slide the box to the goal.}
    \label{fig:bridge-plan} 
\vspace{-2mm}
\end{figure*}

\textbf{Performance on Unseen Physical Reasoning Tasks.}
We evaluate PhyPlan against the baselines based on the minimum regret (defined in Section \ref{sec:problem-formulation}) achieved across five trials taken during the evaluation of the four tasks described in Section \ref{sec:implementation}. After each trial, the task environment is reset to model a C-MAB (Section \ref{sec:problem-formulation}). The lower the regret, the closer the ball gets to the goal and the better the performance. As shown in Figure \ref{fig:regret-results}, PhyPlan consistently achieves lower regret than the baselines. As the task complexity increases, the difference between PhyPlans' performance and the baselines widens. For instance, PhyPlan performs close to the baselines in the Sliding task, whereas it outperforms them by a high margin in the Bridge task.
Figure \ref{fig:dqn-comp} shows a qualitative comparison between PhyPlan and DQN in the \emph{Bridge} task. PhyPlan demonstrates the capability of long-horizon reasoning in substantially less number of trials. PhyPlan has a more structured plan than DQN due to its MCTS-based exploration.

\setcounter{figure}{6}
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Images/result/Qualitative/DQN-vs-PhyPlan_Bridge.PNG}
    \caption{\textbf{Comparing PhyPlan with DQN.} The actions performed by DQN vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
    \label{fig:dqn-comp}
    \vspace{-2mm}
\end{figure}

% \begin{figure*}[t]
% \centering
% \def\imgwidth{0.19\linewidth}
% % \renewcommand*{\thesubfigure}{\alph{subfigure}}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/1.png}
%         % \caption{\fontsize{7}{8}\selectfont Launch Task}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/2.png}
%         % \caption{\fontsize{7}{8}\selectfont Pick the bob}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/3.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/4.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/5.png}
%         % \caption{\fontsize{7}{8}\selectfont Final State}
%     \end{subfigure}

% % \vspace{2mm}

% %     \setcounter{subfigure}{0} 
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/1_init_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Bounce Task}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/2_orient_wedge.png}
% %         \caption{\fontsize{7}{8}\selectfont Orienting Wedge}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/3_pick_ball.png}
% %         \caption{\fontsize{7}{8}\selectfont Picking the Ball}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/4_release_ball.png}
% %         \caption{\fontsize{7}{8}\selectfont Releasing the Ball}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/5_final_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Final State}
% %     \end{subfigure}

% % \vspace{2mm}

%     \setcounter{subfigure}{0} 
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/1.png}
%         % \caption{\fontsize{7}{8}\selectfont  Bridge Task}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/2.png}
%         % \caption{\fontsize{7}{8}\selectfont Placing Bridge}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/3.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/4.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/5.png}
%         % \caption{\fontsize{7}{8}\selectfont Final State}
%     \end{subfigure}

% % \vspace{2mm}

% %     \setcounter{subfigure}{0} 
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/1_init_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Initial State}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/2_adjust_plane.png}
% %         \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/3_adjust_angle.png}
% %         \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, height=0.67\linewidth, frame]{Images/result/Qualitative/Slide Plan/4_release_bob.png}
% %         \caption{\fontsize{7}{8}\selectfont Releasing the Pendulum}
% %     \end{subfigure}

% % \vspace{2mm}

% \caption{\textbf{Simulated Robot Demonstrations.} Physical reasoning tasks learnt by a robot. See videos submitted in the supplementary material.   
% \textbf{LAUNCH:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to throw the ball into the box.
% % \textbf{BOUNCE:} After 3 actions and 10 PINN-rollouts per action, the robot learns to align the wedge correctly and releases the ball at an appropriate height to bounce it into the box.
% \textbf{BRIDGE:} After 5 actions and 20 PINN-rollouts per action, the robot learns to place the bridge in the path of the box and releases the pendulum from the correct location to slide the box to the goal.
% % \textbf{SLIDE:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to slide the puck to the goal.
% }
% \label{fig:task-plan}
% \end{figure*}

\begin{table}[h]
    \centering
    \begin{tabular}{|p{1.6cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|}
        \hline
        \multirow{2}{.3\linewidth}{Models} & \multicolumn{4}{c|}{Regret} \\
        \cline{2-5}& Launch & Bounce & Slide & Bridge \\
        \specialrule{.2em}{.1em}{.01em}
        PhyPlan & 0.09 $\pm$ 0.06 & 0.15 $\pm$ 0.07 & 0.03 $\pm$ 0.02 & 0.09 $\pm$ 0.07 \\
        \hline
        PhyPlan - No Perception & \textbf{0.08 $\pm$ 0.03} & \textbf{0.10 $\pm$ 0.06} & \textbf{0.02 $\pm$ 0.02} & \textbf{0.08 $\pm$ 0.06} \\
        \hline
    \end{tabular}
    \caption{\textbf{Effect of Perception:} Comparing final regret values after five trials by PhyPlan with and without perception. Perception degrades regret by $\sim 10-50\%$ varying with task.}
    \label{tab:perception}
    \vspace{-1mm}
\end{table}

We also implemented a \emph{PhyPlan - No Perception} planner which uses skills trained on data directly from simulator. It does not use perception to infer goal and ball positions. Table \ref{tab:perception} compares the final regret achieved by the two planners after 5 trials. \emph{PhyPlan - No Perception} performs better than \emph{PhyPlan} because of the inherent noise in Perception-based skill networks and the errors in detecting the object positions.
% However, the regret achieved by PhyPlan - No Perception indicates what PhyPlan can achieve if the perception-noise is eliminated.

\begin{table}[h]
    \centering
    \begin{tabular}{|p{2.5cm}|p{1.1cm}|p{1cm}|p{1cm}|p{1cm}|}
    \hline
        \multirow{2}{.3\linewidth}{Models} & \multicolumn{4}{c|}{Time (seconds)} \\
        \cline{2-5}
         & Bridge & Launch & Slide & Bounce \\
        \specialrule{.2em}{.1em}{.01em}
        With High-fidelity simulator & 181.89 $\pm$ 102.08 & 57.13 $\pm$ 34.36 & 30.98 $\pm$ 15.46 & 115.18 $\pm$ 53.41 \\
        \hline
        With Low-fidelity skill model (PhyPlan) & \textbf{35 $\pm$ 0.6} & \textbf{3.8 $\pm$ 0.2} & \textbf{3.07 $\pm$ 0.15} & \textbf{7.75 $\pm$ 1.14} \\
        \hline
    \end{tabular}
    \caption{\textbf{Runtime Comparison.} PhyPlan's runtime is manifold less than the planner without Physics-Informed skill networks that uses a high-fidelity simulator for every rollout.}
    \label{tab:time-results}
    \vspace{-4mm}
\end{table}

Further, Table \ref{tab:time-results} compares PhyPlan with a full simulation engine during planning instead of learnt skills. PhyPlan achieves significant runtime gains (reducing calls to the time-consuming simulator) without losing the task-solving ability.

% \begin{table*}[]
%     \centering
%     \begin{tabular}{|p{3.2cm}|p{1.35cm}|p{1.35cm}|p{1.25cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|}
%         \hline
%         \multirow{2}{.3\linewidth}{Regret} & \multicolumn{2}{c|}{Task: Launch} & \multicolumn{2}{c|}{Task: Bounce} & \multicolumn{2}{c|}{Task: Slide} & \multicolumn{2}{c|}{Task: Bridge} \\
%         \cline{2-9}
%          & Trial 1 & Trial 5 & Trial 1 & Trial 5 & Trial 1 & Trial 5 & Trial 1 & Trial 5 \\
%         \specialrule{.2em}{.1em}{.01em}
%         PhyPlan & 0.14 $\pm$ 0.11 & 0.09 $\pm$ 0.06 & 0.3 $\pm$ 0.09 & 0.15 $\pm$ 0.07 & \textbf{0.08 $\pm$ 0.05} & \textbf{0.03 $\pm$ 0.02} & 0.25 $\pm$ 0.26 & 0.09 $\pm$ 0.07 \\
%         \hline
%         PhyPlan Without Perception & \textbf{0.13 $\pm$ 0.06} & \textbf{0.08 $\pm$ 0.03} & \textbf{0.2 $\pm$ 0.04} & \textbf{0.1 $\pm$ 0.06} & 0.14 $\pm$ 0.04 & 0.1 $\pm$ 0.03 & \textbf{0.15 $\pm$ 0.11} & \textbf{0.11 $\pm$ 0.09} \\
%         \hline
%     \end{tabular}
%     \caption{\textbf{Task Solving Accuracy Without Perception:} PhyPlan without perception generally improves accuracy by $\sim 10-50\%$ depending on the task. The trend reverses for Slide Task and we attribute it to the fact that skill models trained on perceived data are more generalizable and because sliding is a simple skill, they predict the trajectory better.}
%     \label{tab:time-results}
%     \vspace{-1mm}
% \end{table*} 

\textbf{Adaption of Reward Model.}
We also evaluated the effectiveness of GP in adapting to the task execution environment. We create \emph{PhyPlan-No Adapt} same as PhyPlan except the GP online adaptation framework. Figure \ref{fig:online-learning} illustrates the final positions where the dynamic object (the ball) lands relative to the goal after each trial in \emph{Bounce} task. The Random model spans the whole action space, the \emph{DQN-No Adapt} is skewed as it does not learn online, the \emph{DQN} converges to the goal position in later iterations, \emph{PhyPlan-No Adapt} does not explore as it does not learn the prediction error, and \emph{PhyPlan} (with GP) learns the prediction error to converge to the goal position quickly. Further, \emph{PhyPlan} learns more systematically, exploring and refining within a confined action space as also observed in Figure \ref{fig:dqn-comp}.

Figures \ref{fig:pendulum-plan} and \ref{fig:bridge-plan} demonstrate a simulated Franka Emika robot learning to perform the tasks. The robot interacts with the objects using crane grasping with a task space controller for trajectory tracking. The Figure shows the robot learning
% (i) the ball's release height and the wedge's pose in \emph{Bounce} task;
(i) the pendulum's plane and angle in the \emph{Launch} and the \emph{Bridge} tasks; and
(ii) the bridge's pose in the \emph{Bridge} task for the ball or puck to fall into the goal region.
The policy is learnt jointly for all objects, and the actions are delegated to the robot with the desired object in its kinematic range. Once the robots position the tools, the ball or the pendulum is dropped. Further, note that the robot learns to use the bridge effectively; a physical reasoning task reported earlier \cite{allen2020rapid} to be challenging to learn for model-free methods, highlighting the PhyPlan's adaptability to long-horizon tasks. The results indicate the ability to generalise to new goal locations by using objects in the environments to aid task success.
%The results are best viewed as a video submitted as a multi-media supplement to this manuscript. 


==> sections/evaluation-results.tex <==
Through our evaluation, we investigate: i) the ability and efficiency of physics-informed skill networks to model different skills and adapt to unknown physical parameter settings ii) the degree to which our approach can generalize to solving unseen tasks using composition of learnt skills and iii) the qualitative insights and performance of Franka Emika Robot on different physical reasoning tasks.

\setcounter{figure}{3}
\begin{figure*}[tb]
\centering
\def\imgwidth{0.245\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/pendulum.png}
\includegraphics[width=\imgwidth]{Images/result/Task/wedge.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding.png}
\includegraphics[width=\imgwidth]{Images/result/Task/sliding_bridge.png}
\caption{\textbf{Performance on Unseen Tasks:} Comparing our approach and the baselines based on the minimum regret achieved vs the number of trials taken in the evaluation phase for each task. Lower is better. \emph{DQN - No Adapt} does not learn the adapt online. \emph{DQN} and \emph{PhyPlan} both use Gaussian Process for online learning. PhyPlan achieves the lowest regret consistently.}
\label{fig:regret-results}
% \vspace{3mm}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \begin{minipage}[t]{.57\textwidth}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/Wedge_3.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_0.5.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_0.75.png}}
%         \end{subfigure}
%         \begin{subfigure}{0.49\linewidth}
%             {\includegraphics[width=\linewidth, height=0.855\linewidth, frame]{Images/setup/bounce_chain_1.png}}
%         \end{subfigure}
%         \caption{Showing position of the ball predicted by a chain of skill networks at various time steps at a gap of 0.01 seconds ($t_{query}$) in \emph{Bounce} Task. The agent varies the initial drop height (here $0.5, 0.75\ and\ 1.0$) and expects the final resting position of the ball to evaluate the reward.}
%         \label{fig:bounce_chain}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[t]{.42\textwidth}
%         \includegraphics[width=\linewidth]{Images/result/Qualitative/DQN-vs-PhyPlan_Bridge.PNG}
%         \caption{\textbf{Comparing PhyPlan with DQN-Adaptive.} Showing the actions performed by DQN-Adaptive vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use the bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
%         \label{fig:dqn-comp}
%     \end{minipage}
% \end{figure*}

% \begin{figure*}[tb]
% \centering
% \def\imgwidth{0.325\linewidth}
%     \setcounter{subfigure}{0}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-1.png}
%         \caption{DQN-Adaptive: Trial 1}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-4.png}
%         \caption{DQN-Adaptive: Trial 4}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.65\linewidth, frame]{Images/result/Qualitative/Baseline/DQN-11.png}
%         \caption{DQN-Adaptive: Trial 11}
%     \end{subfigure}
%     \setcounter{subfigure}{0}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/1.png}
%         \caption{PhyPlan: Trial 1}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Bridge/2.png}
%         \caption{PhyPlan: Trial 2}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.687\linewidth, frame]{Images/result/Qualitative/Bridge/4.png}
%         \caption{PhyPlan: Trial 4}
%     \end{subfigure}
%     \caption{\textbf{Comparing PhyPlan with DQN-Adaptive.} Showing the actions performed by DQN-Adaptive vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use the bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
%     \label{fig:dqn-comp}
% % \vspace{3mm}
% \end{figure*}

% \begin{figure*}[tb]
% \centering
% \def\imgwidth{0.33\linewidth}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_Random_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Simple_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_Adaptive_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_Without_GP-UCB_wedge_2.PNG}
% \includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_With_GP-UCB_wedge_2.PNG}
% \caption{\textbf{Visual Adaption of Reward Model:} Showing the coordinates of the goal and the ball for 50 iterations. Online Learning explores the action space exhaustively and converges to the optimal action by capturing the systematic errors made by the pre-trained models.}
% \label{fig:online-learning}
% \end{figure*}

\subsection{Evaluation of Learnt Skills} 
We evaluate the prediction accuracy of the proposed physics-informed skill networks on simulation data and the physical parameter estimation in unknown environments.

\textbf{Comparison with baselines} The proposed models: \textit{Physics-Informed Neural Network} a) \textit{with perception} and b) \textit{without perception} are compared against baselines: standard Feedforward network (NN) (same architecture but with only data-driven loss) (a) with perception and (b) without perception. Figure \ref{fig:skill-model} indicates that the model with \textbf{only physics loss} performs poorly due to noise in system, and incorporating physics governing equations with the data loss allows stronger generalisation and improved data efficiency compared to general \emph{physics-uninformed or data only} time series models. PINN without perception is the most efficient skill-learning model. Although performance degrades with perception-based training due to inherent noise in the data, Perception PINN performs better than Perception NN.

\begin{figure}[h]
    \centering
        \includegraphics[width=0.5\linewidth]{Images/result/Quantitative/bar_plot_final.png}
        \includegraphics[width=0.48\linewidth, height=0.425\linewidth]{Images/result/Quantitative/bar_col_plot_final.png}
        \caption{\textbf{Skill Network Accuracy.} Comparing prediction loss on validation dataset. \textbf{Left:} PINN (Physics and Data) without perception performs better than other networks due to the guiding physics and exact data. Physics has less impact in perception-based pipeline due to inherent noise. \textbf{Right:} NN without perception performs better than NN with perception.}
        \label{fig:skill-model}
        % \vspace{1mm}
\end{figure}

\textbf{Adaptiveness to unseen and variable physical parameters} PINN-based skill networks are particularly useful and efficient when the inherent variables of the environment are unknown, as depicted by Figure \ref{fig:unknown}. PINNs are data efficient, which is highlighted by the fact that it requires few steps to determine the actual $\mu$ value accurately. Note even though the perception-based approach is inherently noisy, there is a meagre difference between predicted $\mu$ values by PINN models with and without perception, depicting the robustness of our perception-based approach.

\subsection{Evaluation on Physical Reasoning Tasks}
\textbf{Baselines.}
We implemented the following baselines for comparisons:\footnote{As noted in~\cite{bakhtin2019phyre} policy based learners: A2C~\cite{mnih2016asynchronous} and PPO~\cite{schulman2017proximal} perform poorly as compared to random baseline due to poor training stability hence Deep Q Networks and Random baselines are preferred for evaluation.}
(i) \emph{Random policy:} actions sampled uniformly at random, 
(ii) \emph{DQN-No Adapt:} a DQN baseline from \cite{bakhtin2019phyre} trained using random contexts (images) and random action, reward pairs. The policy is extracted by selecting the highest scoring actions by sampling $10,000$ actions randomly and
(iii) \emph{DQN}: similar to (ii) except, it uses a Gaussian Process to regress over rewards from prior rollouts, as we do in PhyPlan.

\begin{figure}[h]
\centering
\includegraphics[width=0.51\linewidth]{Images/result/PINN/sliding_unknown_new.png}
\includegraphics[width=0.47\linewidth]{Images/result/PINN/distance_plot.png}
        \caption{\textbf{Left: Unknown Parameter} Estimating $\mu$ in \textit{sliding skill}, PINN-based approach achieves a relatively low error within a few time steps. \textbf{Right:} \emph{Generalizing} on variable parameters, PINN is able to accurately predict trajectory of box sliding on surface with variable $\mu$, hence it is efficient.}
        \label{fig:unknown}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Images/result/Qualitative/DQN-vs-PhyPlan_Bridge.PNG}
    \caption{\textbf{Comparing PhyPlan with DQN.} The actions performed by DQN vs those performed by PhyPlan in \emph{Bridge} task. DQN does not use bridge even after 11 actions unlike PhyPlan which uses it starting from the second action and perfectly aligns it in the fourth action to achieve the goal.}
    \label{fig:dqn-comp}
    \vspace{-3mm}
\end{figure}

\begin{figure*}[tb]
\centering
\def\imgwidth{0.195\linewidth}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_Random_wedge_2.PNG}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN - No Adapt_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_DQN_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan - No Adapt_wedge_2.png}
\includegraphics[width=\imgwidth]{Images/result/Task/heat_map_PhyPlan_wedge_2.png}
\caption{\textbf{Effect of GP-based adaptation of reward distribution:} Showing the ball's coordinates relative to the goal for 50 iterations. Online Learning explores the action space exhaustively and converges to the optimal action by capturing the systematic errors made by the pre-trained skill networks.}
\label{fig:online-learning}
% \vspace{3mm}
\end{figure*}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/1.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/2.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/3.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/4.png}
    \includegraphics[width=0.19\linewidth, height=0.1\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/5.png}
    \caption{\textbf{Simulated Robot Demonstrations for Launch Task.} After 2 trials and 10 PINN-rollouts per trial, the robot learns to correctly align the pendulum's plane and angle to throw the ball into the box.}
    \label{fig:pendulum-plan}
\end{figure*}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/1.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/2.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/3.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/4.png}
    \includegraphics[width=0.19\linewidth, height=0.13\linewidth, frame]{Images/result/Qualitative/Bridge Plan/5.png}
    \caption{\textbf{Simulated Robot Demonstrations for Bridge Task.} After 5 trials and 20 PINN-rollouts per trial, the robot learns to place the bridge in the path of the box and releases the pendulum from the correct location to slide the box to the goal.}
    \label{fig:bridge-plan} 
\end{figure*}

\textbf{Performance on Unseen Physical Reasoning Tasks.}
We evaluate PhyPlan against the baselines based on the minimum regret (defined in Section \ref{sec:problem-formulation}) achieved across five trials taken during the evaluation of the four tasks described in Section \ref{sec:implementation}. After each trial, the task environment is reset to model a C-MAB (Section \ref{sec:problem-formulation}). The lower the regret, the closer the ball gets to the goal and the better the performance. As shown in Figure \ref{fig:regret-results}, PhyPlan consistently achieves lower regret than the baselines. As the task complexity increases, the difference between PhyPlans' performance and the baselines widens. For instance, PhyPlan performs close to the baselines in the Sliding task, whereas it outperforms them by a high margin in the Bridge task.
Figure \ref{fig:dqn-comp} shows a qualitative comparison between PhyPlan and DQN in the \emph{Bridge} task. PhyPlan demonstrates the capability of long-horizon reasoning in substantially less number of trials. PhyPlan has a more structured plan than DQN due to its MCTS-based exploration.

% \begin{figure*}[t]
% \centering
% \def\imgwidth{0.19\linewidth}
% % \renewcommand*{\thesubfigure}{\alph{subfigure}}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/1.png}
%         % \caption{\fontsize{7}{8}\selectfont Launch Task}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/2.png}
%         % \caption{\fontsize{7}{8}\selectfont Pick the bob}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/3.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/4.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.55\linewidth, frame]{Images/result/Qualitative/Pendulum Plan/5.png}
%         % \caption{\fontsize{7}{8}\selectfont Final State}
%     \end{subfigure}

% % \vspace{2mm}

% %     \setcounter{subfigure}{0} 
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/1_init_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Bounce Task}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/2_orient_wedge.png}
% %         \caption{\fontsize{7}{8}\selectfont Orienting Wedge}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/3_pick_ball.png}
% %         \caption{\fontsize{7}{8}\selectfont Picking the Ball}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/4_release_ball.png}
% %         \caption{\fontsize{7}{8}\selectfont Releasing the Ball}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Wedge Plan/5_final_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Final State}
% %     \end{subfigure}

% % \vspace{2mm}

%     \setcounter{subfigure}{0} 
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/1.png}
%         % \caption{\fontsize{7}{8}\selectfont  Bridge Task}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/2.png}
%         % \caption{\fontsize{7}{8}\selectfont Placing Bridge}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/3.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/4.png}
%         % \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
%     \end{subfigure}
%     \begin{subfigure}{\imgwidth}
%         \includegraphics[width=\linewidth, height=0.7\linewidth, frame]{Images/result/Qualitative/Bridge Plan/5.png}
%         % \caption{\fontsize{7}{8}\selectfont Final State}
%     \end{subfigure}

% % \vspace{2mm}

% %     \setcounter{subfigure}{0} 
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/1_init_state.png}
% %         \caption{\fontsize{7}{8}\selectfont Initial State}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/2_adjust_plane.png}
% %         \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Plane}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, frame]{Images/result/Qualitative/Slide Plan/3_adjust_angle.png}
% %         \caption{\fontsize{7}{8}\selectfont Adjusting Pendulum Angle}
% %     \end{subfigure}
% %     \begin{subfigure}{\imgwidth}
% %         \includegraphics[width=\linewidth, height=0.67\linewidth, frame]{Images/result/Qualitative/Slide Plan/4_release_bob.png}
% %         \caption{\fontsize{7}{8}\selectfont Releasing the Pendulum}
% %     \end{subfigure}

% % \vspace{2mm}

% \caption{\textbf{Simulated Robot Demonstrations.} Physical reasoning tasks learnt by a robot. See videos submitted in the supplementary material.   
% \textbf{LAUNCH:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to throw the ball into the box.
% % \textbf{BOUNCE:} After 3 actions and 10 PINN-rollouts per action, the robot learns to align the wedge correctly and releases the ball at an appropriate height to bounce it into the box.
% \textbf{BRIDGE:} After 5 actions and 20 PINN-rollouts per action, the robot learns to place the bridge in the path of the box and releases the pendulum from the correct location to slide the box to the goal.
% % \textbf{SLIDE:} After 2 actions and 10 PINN-rollouts per action, the robot learns to correctly align the pendulum's plane and angle to slide the puck to the goal.
% }
% \label{fig:task-plan}
% \end{figure*}

\begin{table}[h]
    \centering
    \begin{tabular}{|p{1.5cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|}
        \hline
        Regret & Launch & Bounce & Slide & Bridge \\
        \specialrule{.2em}{.1em}{.01em}
        PhyPlan & 0.09 $\pm$ 0.06 & 0.15 $\pm$ 0.07 & 0.03 $\pm$ 0.02 & 0.09 $\pm$ 0.07 \\
        \hline
        PhyPlan -No Perception & \textbf{0.08 $\pm$ 0.03} & \textbf{0.10 $\pm$ 0.06} & \textbf{0.02 $\pm$ 0.02} & \textbf{0.08 $\pm$ 0.06} \\
        \hline
    \end{tabular}
    \caption{\textbf{Effect of Perception:} Comparing final regret values after five trials by PhyPlan with and without perception. Perception degrades regret by $\sim 10-50\%$ varying with task.}
    \label{tab:perception}
    % \vspace{-1mm}
\end{table}

We also implemented a \emph{PhyPlan - No Perception} planner which uses skills trained on data directly received from simulator. It does not use perception to infer goal and ball positions. Table \ref{tab:perception} compares the final regret achieved by the two planners after five trials. \emph{PhyPlan - No Perception} performs better than \emph{PhyPlan} because of the inherent noise in the Perception-based skill networks and the errors in detecting the object positions. The regret achieved by PhyPlan - No Perception, however, indicates what PhyPlan can achieve if the perception-noise is eliminated completely.

Further, Table \ref{tab:time-results} compares PhyPlan with a full simulation engine during planning instead of learnt skills. PhyPlan achieves significant runtime gains (reducing calls to the time-consuming simulator) without losing the task-solving ability.

% \begin{table*}[]
%     \centering
%     \begin{tabular}{|p{3.2cm}|p{1.35cm}|p{1.35cm}|p{1.25cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|p{1.35cm}|}
%         \hline
%         \multirow{2}{.3\linewidth}{Regret} & \multicolumn{2}{c|}{Task: Launch} & \multicolumn{2}{c|}{Task: Bounce} & \multicolumn{2}{c|}{Task: Slide} & \multicolumn{2}{c|}{Task: Bridge} \\
%         \cline{2-9}
%          & Trial 1 & Trial 5 & Trial 1 & Trial 5 & Trial 1 & Trial 5 & Trial 1 & Trial 5 \\
%         \specialrule{.2em}{.1em}{.01em}
%         PhyPlan & 0.14 $\pm$ 0.11 & 0.09 $\pm$ 0.06 & 0.3 $\pm$ 0.09 & 0.15 $\pm$ 0.07 & \textbf{0.08 $\pm$ 0.05} & \textbf{0.03 $\pm$ 0.02} & 0.25 $\pm$ 0.26 & 0.09 $\pm$ 0.07 \\
%         \hline
%         PhyPlan Without Perception & \textbf{0.13 $\pm$ 0.06} & \textbf{0.08 $\pm$ 0.03} & \textbf{0.2 $\pm$ 0.04} & \textbf{0.1 $\pm$ 0.06} & 0.14 $\pm$ 0.04 & 0.1 $\pm$ 0.03 & \textbf{0.15 $\pm$ 0.11} & \textbf{0.11 $\pm$ 0.09} \\
%         \hline
%     \end{tabular}
%     \caption{\textbf{Task Solving Accuracy Without Perception:} PhyPlan without perception generally improves accuracy by $\sim 10-50\%$ depending on the task. The trend reverses for Slide Task and we attribute it to the fact that skill models trained on perceived data are more generalizable and because sliding is a simple skill, they predict the trajectory better.}
%     \label{tab:time-results}
%     \vspace{-1mm}
% \end{table*} 

\begin{table}[h]
    \centering
    \begin{tabular}{|p{2.5cm}|p{1.1cm}|p{1cm}|p{1cm}|p{1cm}|}
    \hline
        \multirow{2}{.3\linewidth}{Models} & \multicolumn{4}{c|}{Time (seconds)} \\
        \cline{2-5}
         & Bridge & Launch & Slide & Bounce \\
        \specialrule{.2em}{.1em}{.01em}
        With High-fidelity simulator & 181.89 $\pm$ 102.08 & 57.13 $\pm$ 34.36 & 30.98 $\pm$ 15.46 & 115.18 $\pm$ 53.41 \\
        \hline
        With Low-fidelity skill model (PhyPlan) & \textbf{35 $\pm$ 0.6} & \textbf{3.8 $\pm$ 0.2} & \textbf{3.07 $\pm$ 0.15} & \textbf{7.75 $\pm$ 1.14} \\
        \hline
    \end{tabular}
    \caption{\textbf{Runtime Comparison.} PhyPlan's runtime is manifold less than the planner without Physics-Informed skill networks that uses a high-fidelity simulator for every rollout.}
    \label{tab:time-results}
    \vspace{-4mm}
\end{table}
\textbf{Adaption of Reward Model.}
We also evaluated the effectiveness of GP in adapting to the task execution environment. We create \emph{PhyPlan-No Adapt} same as PhyPlan except the GP online adaptation framework. Figure \ref{fig:online-learning} illustrates the final positions where the dynamic object (the ball) lands relative to the goal after each trial in \emph{Bounce} task. The Random model spans the whole action space, the \emph{DQN-No Adapt} is skewed as it does not learn online, the \emph{DQN} converges to the goal position in later iterations, \emph{PhyPlan-No Adapt} does not explore as it does not learn the prediction error, and \emph{PhyPlan} (with GP) learns the prediction error to converge to the goal position quickly. Further, \emph{PhyPlan} learns more systematically, exploring and refining within a confined action space as also observed in Figure \ref{fig:dqn-comp}.

Figures \ref{fig:pendulum-plan} and \ref{fig:bridge-plan} demonstrate a simulated Franka Emika robot learning to perform the tasks. The robot interacts with the objects using crane grasping with a task space controller for trajectory tracking. The Figure shows the robot learning
% (i) the ball's release height and the wedge's pose in \emph{Bounce} task;
(i) the pendulum's plane and angle in the \emph{Launch} and the \emph{Bridge} tasks; and
(ii) the bridge's pose in the \emph{Bridge} task for the ball or puck to fall into the goal region.
The policy is learnt jointly for all objects, and the actions are delegated to the robot with the desired object in its kinematic range. Once the robots position the tools, the ball or the pendulum is dropped. Further, note that the robot learns to use the bridge effectively; a physical reasoning task reported earlier \cite{allen2020rapid} to be challenging to learn for model-free methods, highlighting the PhyPlan's adaptability to long-horizon tasks. The results indicate the ability to generalise to new goal locations by using objects in the environments to aid task success.
%The results are best viewed as a video submitted as a multi-media supplement to this manuscript. 


==> sections/implementation.tex <==
Our methodology develops offline physics informed skill networks (for different fundamental skills) that can later be used as skill library to be composed together to solve unseen tasks. We created four benchmark tasks: \emph{Launch}, \emph{Slide}, \emph{Bounce}, and \emph{Bridge} (Figure \ref{fig:skill-chaining}).

\textbf{Simulation Platform:} We deploy Nvidia Isaac Gym ~\cite{nvidia2022isaacgym}, a physics simulator and reinforcement learning framework for skill learning and developing the Physical Reasoning Tasks. Skill learning involves simulation-based training, where each skill is simulated, and a physics-informed skill network is trained on the obtained data such as velocity-displacement pair values of the projectile at different times.
% Unseen tasks, exemplified in ~\cite{nvidia2022isaacgym}, demand sequential application of learned physical skills by the robot to achieve defined goals.
% Skill learning involved each skill being simulated, and a physics-informed skill network is trained over the data received. Consider the case of throwing a ball in the simulator, which provides velocity-displacement pair values of the projectile at different time instances as training input. Various unseen tasks are implemented in ~\cite{nvidia2022isaacgym} which require the robot to use physical skills sequentially to attain the goal. For example the Bridge task requires a dynamic object like a ball to be positioned into a goal region. 

\textbf{Object Detection Pipeline:}
Data for Skill Learning is collected via Perception-based pipeline to infer the object state directly from RGB-D data to replicate real lab-based settings. The experimentation scene is captured via an inbuilt depth camera, which provides time series images of skill on which segmentation techniques like unsupervised detection methods (specifically Segment Anything~\cite{kirillov2023segment}, Grounding Dino~\cite{liu2023grounding}) and traditional methods like edge detection are applied. Similarly, while planning on unseen tasks, the robot only observes an image of the scene and infers the initial location of each object (static like goal or dynamic like ball) using \emph{perception}. The robot can then interact with dynamic objects to achieve the goal in generalized configurations.
 % Data for Skill Learning is collected via two approaches: i) Ground Truth approach or Gold Pipeline that directly receives data e.g. velocity of object via ~\cite{nvidia2022isaacgym}. ii) Perception-based pipeline to infer the object state directly from RGB-D data to replicate real lab-based settings. The experimentation scene is captured via an inbuilt depth camera, which provides time series images of skill on which segmentation techniques like unsupervised detection methods like Segment Anything~\cite{kirillov2023segment}, Grounding Dino~\cite{liu2023grounding} and traditional methods like edge detection are applied. For physical reasoning tasks too similar methodologies are applied robot receives data directly from simulator or it only observes an image of the scene with initial placement of each object (static like goal or dynamic like ball) unknown to robot. Perception is used to infer each object's location. The robot can then interact with dynamic objects for achieving goal in generalized configurations.

\textbf{Training Details:}
We train Physics-Informed Neural Networks for each skill (described earlier).
% Based on different dataset collection regimes employed for skill learning two \textbf{Physics-Informed Neural Network} (Figure \ref{fig:motivation}) are trained: \textbf{i) with perception} (Perception-based pipeline), and \textbf{ii) without perception} (Gold Pipeline).
The network architecture comprises of 8 fully connected hidden layers with 40 neurons per layer. We consider actual data points and collocation points (4 times the data points) to optimise the physics-based loss and data-driven loss, respectively. Further, L-BFGS optimizer is used with Xavier normal initialization. 

% Within each rollout the robot can perform multiple trials. In a given trial robot can perform the task of releasing the main dynamic object (say ball) only once after which intial configuration is restored. 

% \begin{figure} 
%     \centering
%     \subfloat[]{\includegraphics[width=0.3\linewidth]{Images/segmentation/projectile_combined.png}}
%     \subfloat[]{\includegraphics[width=0.3\linewidth]{Images/segmentation/goal_wedge_seg.png}}
%     \subfloat[]{\includegraphics[width=0.3\linewidth]{Images/segmentation/ball_sliding_bridge_seg.png}}
%     \caption{\textbf{Perception-based object detection pipeline:} Bounding box along with confidence level for detecting (a) ball being thrown and sliding box, to learn skills, (b) wedge, goal, ball in bounce task, and (c) goal, bridge, table in bridge task, for task inference.}
%     \label{fig:mcts-exp-perception}
% \end{figure}

==> sections/planning.tex <==
% The skill models developed so far allow the robot to predict how the object's trajectory will evolve during a dynamic physical interaction. This can be viewed as \emph{single-step} reasoning.
We formalize the approach to multi-step reasoning by sequentially chaining learnt skills (Figure \ref{fig:skill-chaining}). Utilizing task-specific skill networks, we predict environmental states after executing each skill, culminating in the final state. Evaluation of this final state measures proximity to the goal, demonstrating the effectiveness of our approach for complex task-solving in robot autonomy.
The PINN-predicted trajectories are approximate and semantically evaluate the quality of an action sequence without involving the simulator.

\begin{algorithm}[tb]
    \small
    \caption{\textbf{: Physical-Informed MCTS}}
    \label{alg:mcts}
    % \textbf{Input}: $node,\ goal$ \color{violet} \Comment{Each node corresponds to a state} \color{black} \\
    % % % \textbf{Parameter}: Optional list of parameters\\
    % \textbf{Output}: Reward
    \begin{algorithmic}[1] %[1] enables line numbers
    \Procedure{MCTS}{$node,\ goal$}
        % \color{violet} \Comment{MCTS State Expansion} \color{black}
        \If{$node$ is terminal}
            \State \Return \color{blue} $rv \leftarrow$ \texttt{PINN-based Rollout($node,\ goal$)} \color{black}
            % \color{violet} \Comment{Simulation} \color{black}
        \EndIf
        \State $\mathcal{A}$ $\leftarrow$ set of actions sampled at $node$
        \If{$|\mathcal{A}| > \theta$}
            \State $a^* \leftarrow \underset{a \in \mathcal{A}}{argmax} ~ v_a + \alpha \sqrt{(\log{\underset{a \in \mathcal{A}}{\Sigma} n_a})/n_a}$
            % \color{violet} \Comment{Selection} \color{black}
            \State $newNode$ $\leftarrow$ $node$.child($a^*$)
            \State $rv$ $\leftarrow$ \texttt{MCTS}($newNode$, $goal$)
            % \color{violet} \Comment{Backpropogation} \color{black}
            \State $v_{action} \leftarrow (v_{action} \times n_{action} + rv) / (n_{action} + 1)$
            \State $n_{action} \leftarrow n_{action} + 1$
        \Else
            % \State Add $D$ actions from $UnifromBins(node.actionSpace)$ as arms
            \State $\mathcal{A} \leftarrow$ sample $\mathcal{D}$ actions at $node$
            % \color{violet} \Comment{Expansion} \color{black}
            \For {$a \in \mathcal{A}$}
                \State $child \leftarrow$ $node$.child($a$)
                \State \color{blue} $v_a \leftarrow$ \texttt{PINN-based Rollout($child,\ goal$)} \color{black}
                % \color{violet} \Comment{Simulation} \color{black}
                \State $n_a \leftarrow 1$
            \EndFor
            \State \color{blue} $rv \leftarrow$ \texttt{PINN-based Rollout($node,\ goal$)} \color{black}
            % \color{violet} \Comment{Simulation} \color{black}
        \EndIf
        \State \Return $rv$
    % \EndProcedure\\
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
    \small
    \caption{\textbf{: Adaptive Physical Task Planning}}
    \label{alg:reason}
    \begin{algorithmic}[1]
    \Procedure{Plan}{goal, $T$}
        \For {$t \in T$}
            \State $(\mu_t, \sigma_t) \leftarrow GP(\mu_{t-1}, \sigma_{t-1}, h_{t-1})$ \color{violet} \Comment{Adaptation} \color{black}
            \State $r \leftarrow \underset{i\ \leq \mathcal{K}}{\max}$ \texttt{MCTS} (root node, goal) \color{violet} \Comment{Reasoning} \color{black}
            \State $a \leftarrow$ action sequence corresponding to $r$
            \State $r^* \leftarrow$ Reward from \texttt{Execute} $a$
            \State $h_t \leftarrow (a, (r^* - r))$
        \EndFor
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
    \small
    \caption{\textbf{: PINN-based Rollout}}
    \label{alg:rollout}
    \textbf{Input}: $node,\ goal$ \color{violet} \Comment{Each node corresponds to a state} \color{black} \\
    % \textbf{Parameter}: Optional list of parameters\\
    \textbf{Output}: Reward
    \begin{algorithmic}[1] %[1] enables line numbers
        \For{s $\in$ Skill\_Sequence}  \color{violet} \Comment{Skill Chaining} \color{black}
            \State t $\leftarrow$ time\_step
            \State $node \leftarrow PINN_s(PINN_s(\ldots(PINN_s(node, t),\ldots t),t)$
        \EndFor
        \State $r \leftarrow$ evaluate($node,\ goal$)
        \State a $\leftarrow$ sequence of actions corresponding to $r$
        \State $\mu, \sigma \leftarrow$ Gaussian\_Process.predict(a)
        \State \Return \color{blue} rv + $\left(\mu + \beta^{1/2} \times \sigma\right)$ \color{violet} \Comment{Adding GP posterior} \color{black}
    \end{algorithmic}
\end{algorithm}

We assume the chain of skills to perform the tasks, and PhyPlan finds the best action in each skill, such as the angles of the bridge, pendulum's plane and at which to swing the pendulum in \emph{Bridge} task. We run an MCTS planning algorithm (Algorithm \ref{alg:mcts}) with \texttt{PINN-based Rollouts} (Algorithm \ref{alg:rollout}) to search the continuous action space by uniformly sampling $\mathcal{D}$ (Discretization Factor) actions within the bounds of the space. The lines coloured blue in Algorithm \ref{alg:mcts} are where we differ from conventional MCTS. Also, $n_{action}$ and $v_{action}$ are the number of trials and the value of \emph{action}, respectively. The planner (Algorithm \ref{alg:reason}) expands the Monte Carlo Tree for a maximum number of iterations ($\mathcal{K}$) with a typical $\mathcal{D}$ and $\mathcal{K}$ at $20$ and $10$, respectively. Then, it executes the best action according to the skill network in the simulator. However, since the skill networks could make systematic errors, it finetunes the reward predictor by approximating the error as a Gaussian Process (GP). Given $t-1$ samples of action and error pairs, the GP provides a Gaussian posterior $\mathcal{N}(\mu_{t-1}, \sigma_{t-1})$ over the error of the next action $a_t$ for any action in the action space $\mathcal{A}$ \cite{moses2020visual}. The MCTS uses this GP to correct the reward predictor in the search for the next action using the equation $r_t = r_t + \mu_{t-1}(a_t) + \beta^{1/2}\sigma_{t-1}(a_t)$, where $r_t$ is the reward predicted by the skill model, $\mu_{t-1}(a_t)$ and $\sigma_{t-1}(a_t)$ are the mean and variance of the function value at $a_t$ at time $t-1$, and $\beta$ is a hyperparameter; we use $\beta = 0.25$.
 

==> sections/problem_statement.tex <==
We consider a robot manipulator operating in a tabletop environment. Assume that the robot can position its end-effector at a desired configuration, grasp an object, move it while holding it, and release the object-oriented at a target pose. The environment consists of dynamic objects (box/puck/ball) and static objects such as a wedge, a flat surface (such as a table), a positioning plank (for instance, a bridge), a box-like object (goal), a pendulum-like assembly capable of swinging a plan that rotates on a hinge. The dynamic object can interact with other objects, e.g., by sliding over a surface, colliding and rebounding from a wall, or more naturally under gravity (dropping vertically or falling as a projectile), finally coming to rest on a ground surface or inside a container-like object. Formally, let $s_t \in \mathcal{S}$ denote the world state at time $t$, observed as an image $i_t$ from a depth camera. Let $\mathcal{O}$ denote the set of objects in the environment, where each $o \in \mathcal{O}$ has a set of modes, $M(o)$ (degrees of freedom) for interacting with the environment. For example, a wedge may be positioned at a coordinate $(x, y)$ and oriented as $q$, leading to $M(wedge) = \{x, y, q\}$. Similarly, the interaction modes for a pendulum can be the release angle $\theta$ and length $l$. For a projectile, it may be velocity $v$ and height of release $h$. We represent the action taken on state $s_t$ as $a_t \in \mathcal{A}$. Action outcomes are considered non-deterministic and modelled as a stochastic transition model $s_{t+1} \sim T(s_t, a_t)$, arising from execution in the real environment or a realistic physics simulation engine. 

The robot's objective is to ensure that the dynamic object reaches a specified region of space (implicitly defined by a target container). We denote the goal region for the target object as $g$. Direct grasping and releasing the object may not be feasible, particularly when the goal region is far from the object. Hence, the robot may interact with objects as a tool, \textit{i.e.}, position and release points in continuous space, such that when the object is released, the dynamic interactions facilitate reaching goal regions. For instance, a ball resting on a table may be hit by a pendulum, slide on a table, and fall into a target region via projectile motion. The goal regions are embedded in the reward model
$R: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \mapsto \mathbb{R}$.
This translates to a high reward when the object is contained within the goal region and low otherwise. In our setup, we obtain the reward $r_t$ after performing action $a_t$.

We learn a goal-conditioned policy $a_t \sim \pi_g(s_t)$, where $a_t$ is a tuple indicating the setting of interactive variables for each object, such as $a_ t = \{M(o_1), M(o_2), \ldots, M(o_n)\}$. Directly learning this policy is challenging, mainly when the task requires sequential multi-step interaction over time, as this requires long-horizon temporal and causal reasoning as reaching goals with multiple tool-like objects spans a large space of possible trajectories. This work simplifies the long-horizon reasoning by reducing the problem to myopic action optimisation. Here, we take action $a_t$ only based on $s_t$, obtain the reward, update our model, and reset decision-making. Expressly, we set the configuration or interactive variables of the dynamic objects to the desired values and release them. This is considered as a single ``epoch''. We do not consider future states like $s_{t+1}$. Hence, our setup is one of Contextual Multi-armed Bandits (C-MAB)~\cite{lu2010contextual}. Our policy aims to minimise the regret $e = \tfrac{r - r*}{r}$, where $r$ is the maximum reward obtained by the agent in a simulation run, and $r*$ is the theoretical maximum reward. We observe that learning this policy requires time-consuming simulation of actions that slow down the learning process. Hence, we explore ways to accelerate learning using learnt physics simulators.

\setcounter{figure}{2}
\begin{figure*}
    \centering
    % First row of images
    % \begin{minipage}{0.19\linewidth}
    %     \includegraphics[width=\linewidth]{Images/skills/sliding_skill.jpg}
    % \end{minipage}\hfill
    % \begin{minipage}{0.19\linewidth}
    %      \includegraphics[width=\linewidth]{Images/skills/projectile_skill.jpg}
    % \end{minipage}\hfill
    % \begin{minipage}{0.19\linewidth}
    %      \includegraphics[width=\linewidth]{Images/skills/pendulum.jpg}
    % \end{minipage}\hfill
    % \begin{minipage}{0.19\linewidth}
    %     \includegraphics[width=\linewidth]{Images/skills/collision_skill.jpg}
    % \end{minipage}\hfill
    % \begin{minipage}{0.19\linewidth}
    %      \includegraphics[width=\linewidth]{Images/skills/pend_peg.jpg}
    % \end{minipage}
    
    % \vspace{1mm} %  
    
    % Second row of images
    \begin{minipage}{0.24\linewidth}
         \includegraphics[width=\linewidth]{Images/setup/PhyPlan_Design_Launch.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
         \includegraphics[width=\linewidth]{Images/setup/PhyPlan_Design_Bounce.pdf} 
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
         \includegraphics[width=\linewidth]{Images/setup/PhyPlan_Design_Slide.pdf} 
    \end{minipage}\hfill
    \begin{minipage}{0.24\linewidth}
         \includegraphics[width=\linewidth]{Images/setup/PhyPlan_Design_Bridge.pdf}
    \end{minipage}
    \caption{
    % \textbf{Top: Dynamic Physical Skills.} Dynamic interactions by a manipulator we consider in this work. The agent's goal is to compose these skills to perform a high-level unseen task. 
    \textbf{Physical Reasoning Tasks} We considered four tasks: Launch, Bounce, Slide, and Bridge, that require (i) sequential composition of skills (hitting, sliding etc. to get the ball in the goal region) and (ii) generalization (unknown parameters e.g., friction coefficient). The tasks are inspired from benchmarks in  \cite{allen2020rapid,bakhtin2019phyre}; extended to 3D domain with a simulated robot.}
    \label{fig:skill-chaining} 
\end{figure*}

==> sections/skills.tex <==
Instead of learning a policy directly, we factor the learning problem above as one of learning a model that depicts how an object engages with the environment and then using this model to plan multi-step interactions to reach the intended goals. We postulate that a learnt physical interaction model would provide a strong prior for the planner and help them make informed decisions. We consider the problem of learning a model for physical skills such as \emph{bouncing} a ball-like object off a wedge, \emph{sliding} over an object, \emph{swinging} a pendulum, \emph{throwing} an object as a projectile and \emph{hitting} an object with a pendulum. Here, we interpret a physical skill as a model that predicts the state trajectory of an object as it undergoes a dynamic interaction with another object.

Governing physics of such a skill can be represented as $Y_t = g(Y)$, where $Y$ represents the state variables, $Y_t$ represents the time derivative of the state variable, and g(Y) represents a non-linear function of $Y$. For instance, skills like throwing can be modelled as  projectile motion with a governing differential equation: $d^2y/dt^2 + g = 0$ representing motion in the vertical axis and $dx/dt - vx_{init} = 0$ 
representing motion in the horizontal plane. Here, $x$ and $y$ represent instantaneous position w.r.t. inertial frame in the horizontal and vertical direction, respectively, and $vx_{init}$ represents the initial horizontal velocity. Similarly, other skills like swinging can be modelled by pendulum dynamics and sliding as friction dynamics.


We introduce a neural network that predicts the object's state during dynamic interaction continuously parameterised by time (Figure \ref{fig:bounce_chain}). Such interactions can be simulated in a physics engine by using numerical integration schemes. However, since we aim to perform multi-step interactions, simulating outcomes during training is often intractable. Hence, we adopt a learning-based approach and learn a function $f(X, t) \rightarrow Y$ that predicts the object's state during dynamic interaction continuously parameterised by time. We represent $f(X, t)$ with a neural network that trains on $N_u$ number of training data points. We employ a physics-informed loss function or $L_P(\theta)$  to constrain the latent space, which we compute on $N_p$ number of points in latent space referred as collocation points. Here $L_P(\theta) = \left({1/N_f}\right) \sum_{1}^{N_f} ( \mathcal{R}(X_P^i, \theta))^2$, where $\mathcal R (X_P^i, \theta):= \hat{Y}_t - g(\hat{Y}(X_P^i))$ is residual of the governing physics (defined earlier) after inserting neural network output in it, and $X_P^i$ represents the $i^{th}$ collocation point. $\hat Y$ represents the neural network output, and $\hat{Y}_t(X_P^i)$ represents the derivative of the neural network predicted state variable obtained using automatic differentiation. For training the network in practice, we use both physics-based and data-driven loss functions,
$
L(\theta) = L_D(\theta) + L_P(\theta)
$,
where $L_D(\theta) = \left({1/N_u}\right) \sum _{1}^{N_u} ( Y_D^i - NN(X_D^i, \theta))^2
$ is the data driven loss. Figure \ref{fig:motivation} provides the architecture of the Physics-Informed Skill Network. The physics-based loss enables the model to train from a sparse dataset ($N_u << N_f$), enabling rapid skills learning. 
%
In practice, the parameters associated with physics models are not known apriori. For example, the coefficient of friction is often not known. PINN treats the unknown parameter as additional trainable parameters (absorbed in $\theta$) and estimates the same by solving the aforementioned optimisation problem. We use PINN to learn throwing, sliding, and swinging skills, and the trained PINN models are referred to as ``Physics-Informed Skill Networks''. However, collision skills are learnt directly from data because of complex and intractable physics of their motion.
%\footnote{Learning in such settings remains a part of future work}. 
%Figure \ref{fig:skill-learning} shows an example the skill sets considered in this paper.


%% Commenting out the figure for space. May bring back. 
\iffalse
\begin{table*}
    \centering
    \renewcommand{\arraystretch}{1.5} % Adjust the cell spacing
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        Skill & Swinging & Sliding & Throwing & Bouncing & Hitting \\[2pt]
        \specialrule{.2em}{.1em}{.01em}
        Input & $(\theta_{init}, t_{query})$ & $(v_{init}, t_{query})$ & $(v_{{hor}_{init}}, v_{{ver}_{init}}, t_{query})$ & $(e,\theta, v_{{ver}_{init}}, v_{{hor}_{init}})$ & $(m_{1},m_{2}, v_{init})$ \\[2pt]
        \hline
        Output & $(\theta_{query}, \omega_{query})$ & $(x_{query}, v_{query})$ & $(v_{{ver}_{query}}, y_{query}, x_{query})$ & $(v_{{ver}_{query}}, v_{{hor}_{query}})$ &  $v_{query}$ \\[2pt]
        \hline
        ODE & $\frac{d^2\theta}{dt^2} + \frac{g * sin(\theta)}{l} = 0,$ &  $\frac{d^2x}{dt^2} + \mu g = 0,$  & $\frac{v_{{ver}_{init}}}{dt} + g = 0, \frac{d^2y}{d^2t} + g = 0,$  & None &  None \\[2pt]
        
        & $\frac{d\omega}{dt} + \frac{g * sin(\theta)}{l} = 0$  & $ \frac{dv}{dt} + \mu g = 0$ & $ \frac{dx}{dt} - v_{{hor}_{init}} = 0$ &  & \\[2pt]
        \hline
    \end{tabular}
    }
    \caption{\textbf{Skill Network Training details.} Showing the input, output, and governing equations used to train skill networks. $init$ signifies the initial value of a physical parameter, and $t_{query}$ denotes the time instance for which the output quantity is required. $v_{hor}$ and $v_{ver}$ represent planar and vertical velocities, respectively, with the latter directed towards gravity (g).}
    \label{table:Skill-Table}
    % \vspace{2mm}
\end{table*}
\fi
